Autonomous AI Bird Feeder for Backyard Biodiversity Monitoring

This paper presents a low cost, on premise system for autonomous backyard bird monitoring in Belgian urban gardens. A motion triggered IP camera uploads short clips via FTP to a local server, where frames are sampled and birds are localized with Detectron2; cropped regions are then classified by an EfficientNet-B3 model fine tuned on a 40-species Belgian subset derived from a larger Kaggle corpus. All processing runs on commodity hardware without a discrete GPU, preserving privacy and avoiding cloud fees. The physical feeder uses small entry ports (30 mm) to exclude pigeons and reduce nuisance triggers. Detector-guided cropping improves classification accuracy over raw-frame classification. The classifier attains high validation performance on the curated subset (about 99.5 percent) and delivers practical field accuracy (top-1 about 88 percent) on held-out species, demonstrating feasibility for citizen-science-grade biodiversity logging at home.

==> tex/style/commands.tex <==
% Custom commands
\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eqnref}[1]{Eq.~\eqref{eq:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}

% Unicode character definitions
\DeclareUnicodeCharacter{2248}{\ensuremath{\approx}}  % ≈
\DeclareUnicodeCharacter{2192}{\ensuremath{\rightarrow}}  % →
\DeclareUnicodeCharacter{2009}{\,}  % thin space

% Add more custom commands as needed

